De-SaTE: Denoising Self-attention Transformer Encoders for Li-ion Battery Health Prognostics

The usage of Lithium-ion (Li-ion) batteries has gained widespread popularity across various industries, from powering portable electronic devices to propelling electric vehicles and supporting energy storage systems. A central challenge in Li-ion battery reliability lies in accurately predicting their Remaining Useful Life (RUL), which is a critical measure for proactive maintenance and predictive analytics. This study presents a novel approach that harnesses the power of multiple denoising modules, each trained to address specific types of noise commonly encountered in battery data. Specifically, a denoising auto-encoder and a wavelet denoiser are used to generate encoded/decomposed representations, which are subsequently processed through dedicated self-attention transformer encoders. After extensive experimentation on NASA and CALCE data, a broad spectrum of health indicator values are estimated under a set of diverse noise patterns. The reported error metrics on these data are on par with or better than the state-of-the-art reported in recent literature.

==> unnecessary.tex <==
% Ren et al.\cite{30} proposed an Auto-enocoder-Convolutional Neural Network-Long Short Term Memory Model that mines deeper information in finite data by using an Auto-encoder to extract features from raw data and a combination of convolutional and \ac{LSTM} layers to learn temporal patterns in the data. 

% Various deep learning techniques have been proposed for \ac{RUL} estimation, including the LSTM-RNN method proposed by Zhang et al.\cite{25}, which captures long-term temporal dependencies of capacity degradation by using a sequence of memory cells to store past information. Ren et al. \cite{26} proposed an integrated deep learning approach that combines the Auto-encoder with \ac{DNN} to extract multi-dimensional features and estimate \ac{RUL}.


% \iffalse
% Moreover, transformers exhibit a remarkable aptitude for managing the intricacies of multi-modal data sources and vast, high-dimensional datasets. This unique capability empowers them to deliver comprehensive and highly accurate predictions, even in scenarios where diverse and extensive data inputs are involved. In the following sections, we embark on a comprehensive exploration of the transformative power inherent in transformer architectures and their pivotal role in advancing the methodologies employed for \ac{RUL} estimation. 

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=10 cm,height=6 cm, keepaspectratio]{Vanilla Transformer Architecture .png}}
%     \caption{ Vanilla Transformer architecture  }
%     \label{Vanilla Transformer architecture }
% \end{figure}
% Refer \ref{Vanilla Transformer architecture } \cite{81} for Transformer model architecture.
% The transformer architecture comprises two main components: an encoder and a decoder. The encoder processes the input sequence, capturing its contextual information. The decoder, on the other hand, generates output sequences, attending to different parts of the input sequence as needed. This architecture excels at handling sequential data, making it highly effective for tasks like language translation and time-series forecasting.

% \vspace{0.2 cm}
% Mathematically, the transformer \cite{81} architecture is underpinned by a series of intricate equations that orchestrate the encoding and decoding processes. These equations are essential in enabling the model to process sequential data efficiently and capture intricate patterns within it. The following equations succinctly encapsulate the core mathematical operations that power the transformer architecture.

% \vspace{0.2 cm}
% \textbf{Encoder Component:}
% \textbf{Self-Attention Mechanism:}
% The encoder's self-attention mechanism \cite{vaswani_trans} computes attention scores for each position in the input sequence, allowing the model to weigh the importance of different elements in the sequence when encoding a particular position. This is typically computed using a weighted sum:
% \textbf{Equation:}
% \[
% A(Q,K,V) = \text{softmax}\left(\frac{QK^T}{\sqrt{d_k}}\right)V
% \]
% Here,
% \begin{align*}
%     & Q \text{ represents the query matrix for the input sequence.} \\
%     & K \text{ represents the key matrix for the input sequence.} \\
%     & V \text{ represents the value matrix for the input sequence.} \\
%     & d_k \text{ is a scaling factor to stabilize the gradients.}
% \end{align*}

% \vspace{0.1cm}

% \textbf{Multi-Head Attention:}
% The self-attention mechanism is often used in multiple heads to capture different types of dependencies

% \vspace{0.1 cm}
% \textbf{Equation:}
% \[
% \text{MultiHead}(Q,K,V) = \text{Concat}(\text{head}_1, \text{head}_2, ..., \text{head}_h)W^O
% \]

% Here,
% \begin{align*}
%     & \text{head}_i \text{ represents the output of the } i\text{-th attention head.} \\
%     & W^O \text{ is a learnable weight matrix.}
% \end{align*}

% \vspace{0.1cm}

% \textbf{Feed-Forward Network:}
% After attention, the output passes through a feed-forward neural network:

% \vspace{0.1 cm}
% \textbf{ Equation:}
% \[
% \text{FFN}(x) = \text{ReLU}(xW_1+b_1)W_2+b_2
% \]

% Here,
% \begin{align*}
%     & W_1, b_1, W_2, b_2 \text{ are learnable weights and biases.}
% \end{align*}

% \vspace{0.2 cm}
% \textbf{Decoder Component:}

% \vspace{0.1cm}
% \textbf{Masked Self-Attention:}
% In the decoder, self-attention is used with a masking mechanism to prevent positions from attending to future positions:

% \vspace{0.1 cm}
% \textbf{Equation:}
% \[
% A(Q,K,V) = \text{softmax}\left(\frac{QK^T}{\sqrt{d_k}}\odot\text{Mask}\right)V
% \]

% The \(\odot\) symbol denotes element-wise multiplication, and the "Mask" prevents positions from attending to future positions.

% \vspace{0.1 cm}
% \textbf{Encoder-Decoder Attention:}
% The decoder can also attend to the encoder's output:

% \vspace{0.1 cm}
% \textbf{Equation:}
% \[
% A(Q,K,V) = \text{softmax}\left(\frac{QK^T}{\sqrt{d_k}}\right)V
% \]

% \vspace{0.1cm}

% \textbf{Position-wise Feed-Forward Network:}
% The decoder output passes through a position-wise feed-forward network:

% \vspace{0.1 cm}
% \textbf{Equation:}
% \[
% \text{FFN}(x) = \text{ReLU}(xW_1+b_1)W_2+b_2
% \]

% Here,
% \begin{align*}
%     & W_1, b_1, W_2, b_2 \text{ are learnable weights and biases.}
% \end{align*}

% \vspace{0.1 cm}
% In the context of \ac{LIB}, the application of transformer-based models has garnered attention for their potential in enhancing \ac{RUL} prediction. Researchers have started to explore the advantages of transformers in capturing the complex degradation patterns and temporal dependencies inherent in battery data. Notably, Chen et al. \cite{82} demonstrated significant advancements in \ac{RUL} prediction by employing the Denoising Transformer. This novel approach excels in mitigating the impact of input noise, resulting in more accurate and robust predictions. As the field of battery health monitoring continues to evolve, transformer-based variations should be explored to extract valuable insights.

% \begin{table}[h]
% \centering
% \begin{tabular}{|p{1.0cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% \textbf{Method} & \textbf{Accuracy} & \textbf{Forecast cycle percent} & \textbf{Issue}\\
% \hline
% Data Driven & High & Less & Data-Intensive Algorithms\\
% \hline
% Model Based Method & Medium & Many & Complex Modeling\\
% \hline
% \end{tabular}
% \vspace{0.2cm}
% \caption{Comparison of \ac{RUL} estimation methods.}
% \label{table:rul_comparison}
% \end{table}


% \iffalse
% \vspace{0.5cm}
% \section{Industrial Applications}

% Lithium-ion batteries have transcended traditional boundaries and found application across a multitude of sectors, each harnessing their unique attributes for transformative results.Lithium-ion batteries find wide-range applications in the healthcare,transportation,space exploration and consumer electronic sectors.
% \label{key applicastions}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=10 cm,height=20 cm, keepaspectratio]{LIB applications .png}
%     \caption{Lithium Ion Battery Life cycle for Industrial Setting}
%     \label{Lithium Ion Battery Life cycle for Industrial Setting}
% \end{figure}

% Figure \ref{Lithium Ion Battery Life cycle for Industrial Setting} illustrates a commonly adopted strategy for handling lithium-ion batteries within an industrial context.

% \vspace{0.2cm}

% Here's a more concise and refined description of the above figure:

% \begin{itemize}
%     \item \textbf{Battery Icon} : Represents the initial Lithium-Ion battery.
%     \item \textbf{Industrial Applications} : Depict various applications utilizing the battery's power. 
%     \item \textbf{Capacity Degradation Curve} : Illustrates the battery's gradual capacity decline over time.
%     \item \textbf{\ac{RUL} Prediction Approaches} : Data driven and Model based. 
%     \item \textbf{Accuracy vs Complexity Tradeoff} : This is the major factor to be considered while choosing the right \ac{RUL} prediction method based on the industrial sector.
%     \item \textbf{80 percent Alert} : Triggers when the battery's capacity reaches 80 percent of it's original capacity.
%     \item \textbf{Human in loop} : Involves Human Intervention when receiving an alert.
%     \item \textbf{Battery Disposal Decision} : Determines the action to be performed on the battery.
% \end{itemize}

% \vspace{0.2cm}

% The below table serves as an invaluable resource for industrialists seeking to harness the potential of Lithium-Ion batteries within their specific industrial domains. It offers direct access to research papers essential for a comprehensive understanding of RUL (Remaining Useful Life) prediction for Lithium-Ion batteries in various industrial sectors. These papers encompass a wide spectrum of data-driven and model-based approaches, equipping entrepreneurs with the foundational knowledge required to embark on ventures tailored to their industrial contexts.
% \vspace{0.2cm}

% \begin{table}[!ht]
% \centering
% \small % Reduce font size
% \setlength{\tabcolsep}{3pt} % Reduce the column spacing
% \begin{tabular}{|p{1.8 cm}|p{2 cm}|p{2 cm}|p{2 cm}|}
% \hline
% \textbf{Industrial Sector} & \textbf{Applications} & \textbf{Data-Driven} & \textbf{Model-Based} \\
% \hline
% \centering Transportation &Cars,E-bikes,Public Transport &Refer \cite{68} for \ac{ML} approaches.\cite{69} Examines deep learning methodology & Refer \cite{66} for Adaptive Filter approach, refer \cite{67} for Stochastic Process Methods \\
% \hline
% Consumer Electronics & Smartphones, wearable devices & Paper\cite{70} suggests Data Mining approach, refer \cite{71} for \ac{ML} approach & Refer\cite{72} for Statistical approaches\\
% \hline
% Space Exploration & Rovers and communication equipment & Refer\cite{75} for Deep Learning methods, refer\cite{76} for Traditional Machine Learning methods & \cite{73} and \cite{74} discuss Adaptive Filter approaches\\
% \hline
% Healthcare & Implantable medical devices & Refer\cite{79} for Deep Learning method &\cite{77} and \cite{78} use Adaptive Filter approach and Stochastic Processes respectively for \ac{RUL} prediction\\
% \hline
% \end{tabular}
% \vspace{0.2cm}
% \caption{Getting started with Data-driven and Model-based approaches for industrial applications}
% \label{table:GettingStarted}
% \end{table}
% \fi

% \vspace{0.2cm}
% \section{Key Issues}
% \label{Key Issues}

% In the realm of \ac{Li-ion} battery health assessment and \ac{RUL} estimation, some critical challenges must be addressed to ensure the reliability and applicability of such models.

% \vspace{0.2 cm}
% \begin{enumerate}
%     \item \textbf{Data Quality:}
%     \begin{itemize}
%         \item Accurate and complete data are essential for reliable \ac{RUL} predictions.
%         \item Inaccurate or incomplete data can lead to unreliable \ac{RUL} estimates.
%     \end{itemize}
    
%     \item \textbf{Battery Variability:}
%     \begin{itemize}
%         \item Different batteries exhibit varying degradation patterns and deterioration rates.
%         \item Models need to account for this variability to be effective and adaptable.
%     \end{itemize}
    
%     \item \textbf{Model Parameter Selection:}
%     \begin{itemize}
%         \item The accuracy of \ac{RUL} estimates relies heavily on selecting and optimizing model parameters.
%         \item Parameters may differ based on battery chemistry, operational conditions, and external factors.
%     \end{itemize}
    
%     \item \textbf{Consistency and Standardization:}
%     \begin{itemize}
%         \item Lack of consistency and standardization in \ac{RUL} estimation processes hinders comparability.
%         \item Establishing standardized testing techniques and protocols is crucial for reliable results.
%     \end{itemize}
    
%     \item \textbf{Scalability:}
%     \begin{itemize}
%         \item Many existing \ac{RUL} estimation models are designed for small-scale applications.
%         \item Scalable models are needed to address the requirements of large-scale battery systems.
%     \end{itemize}
    
%     \item \textbf{Computational Efficiency:}
%     \begin{itemize}
%         \item Many \ac{RUL} estimation models are computationally intensive, limiting real-time applications.
%         \item Developing computationally efficient models capable of real-time predictions is essential.
%     \end{itemize}
% \end{enumerate}

% \vspace{0.2 cm}
% Addressing these issues is paramount for the development of accurate, dependable, and scalable \ac{RUL} estimation models for \ac{Li-ion} batteries. 
% \fi
